Online Coreset Selection for Rehearsal-based Continual Learning

A dataset is a shred of crucial evidence to describe a task. However, each data point in the dataset does not have the same potential, as some of the data points can be more representative or informative than others. This unequal importance among the data points may have a large impact in rehearsal-based continual learning, where we store a subset of the training examples (coreset) to be replayed later to alleviate catastrophic forgetting. In continual learning, the quality of the samples stored in the coreset directly affects the model's effectiveness and efficiency. The coreset selection problem becomes even more important under realistic settings, such as imbalanced continual learning or noisy data scenarios. To tackle this problem, we propose Online Coreset Selection (OCS), a simple yet effective method that selects the most representative and informative coreset at each iteration and trains them in an online manner. Our proposed method maximizes the model's adaptation to a current dataset while selecting high-affinity samples to past tasks, which directly inhibits catastrophic forgetting. We validate the effectiveness of our coreset selection mechanism over various standard, imbalanced, and noisy datasets against strong continual learning baselines, demonstrating that it improves task adaptation and prevents catastrophic forgetting in a sample-efficient manner.

==> 2_intro_old.tex <==
\section{Introduction}

Humans possess the ability to learn a large number of tasks by accumulating knowledge and skills over time. Building a system resembling human learning abilities is a deep-rooted desire since sustainable learning over a long-term period is essential for general artificial intelligence. In light of this need, \emph{continual learning} (CL)~\citep{ThrunS1995}, or \emph{lifelong learning}, tackles a learning scenario where a model continuously learns over a sequence of tasks~\citep{KumarA2012icml,LiZ2016eccv} within a broad research area, such as classification~\citep{kirkpatrick2017overcoming,chaudhry2018efficient}, image generation~\citep{zhai2019lifelong}, language learning~\citep{li2019compositional, biesialska2020continual}, clinical application~\citep{lee2020clinical, lenga2020continual, baweja2018towards}, speech recognition~\citep{sadhu2020continual}, and federated learning~\citep{yoon2020federated}. A well-known challenge for continual learning is \emph{catastrophic forgetting}~\citep{mccloskey1989catastrophic}, where the continual learner loses the fidelity for past tasks after adapting the previously learned knowledge to future tasks. 

Recent rehearsal-based continual learning methods adapt the continual model to the previous tasks by maintaining and revisiting a small replay buffer~\citep{chaudhry2018efficient,titsias2019functional,mirzadeh2020understanding}. However, the majority of these methods store random-sampled instances as a proxy set to mitigate catastrophic forgetting, limiting their practicality to real-world applications (see ~\Cref{fig:existing_methods}). However, all the training instances are not equally useful, as some of them can be more representative or informative for the target task, and others can lead to performance degeneration for previous tasks. Furthermore, these unequal potentials could be more severe under practical scenarios containing \emph{imbalanced, streaming, or noisy instances} (see ~\Cref{fig:setup}). 
This leads to an essential question in continual learning:

% {In this work, we \sout{primarily} focus on rehearsal-based continual learning for vision tasks.} \TBDD{While the existing rehearsal-based methods learn all arriving data points indiscreetly and memorize samples by considering the current task for standard online/offline continual learning problem, we demonstrate that our proposed method outperforms these approaches across diverse and challenging continual learning settings. our OCS immediately selects the most helpful subset from arriving data streams to update the model and obtains a coreset that further minimizes the interference with past tasks to mitigate the catastrophic forgetting directly.}

\begin{quote}
\centering
\emph{How can we obtain a coreset to promote task adaptation for the current task while minimizing catastrophic forgetting on previously seen tasks?}
\vspace{-0.1in}
\end{quote}
%\input{materials/2_method_compaison_table}
\input{materials/2_concept_figure}
\input{materials/2_noisy_setup} 


To address this question, we propose \emph{Online Coreset Selection (OCS)}, a novel method for continual learning that selects representative training instances for the current and previous tasks based on our following three selection strategies: \textbf{(1)} \emph{Minibatch similarity} selects samples that are representative to the target task $\mathcal{T}_t$. \textbf{(2)} \emph{Cross-batch diversity} encourages minimal redundancy among the samples of target task $\mathcal{T}_t$. \textbf{(3)} \emph{Coreset affinity} promotes minimum interference between the selected samples and knowledge of the previous tasks $\mathcal{T}_k,~\forall k<t$. To this end, OCS minimizes the catastrophic forgetting on the previous tasks by utilizing the obtained coreset for future training, and also encourages the current task adaptation by updating the model parameters on the top-$\kappa$ selected data instances. The overall concept is illustrated in \Cref{fig:ocs_concept}.

Our method is simple, intuitive, and is generally applicable to any rehearsal-based continual learning method. We evaluate the performance of OCS on various continual learning scenarios and show that it outperforms state-of-the-art rehearsal-based techniques on balanced, imbalanced, and noisy continual learning benchmarks of varying complexity. We also show that OCS is general and exhibits collaborative learning with the existing rehearsal-based methods, leading to increased task adaptation and inhibiting catastrophic forgetting. To summarize, our contributions are threefold:
\begin{itemize}[leftmargin=1.2em, partopsep=0em]
\item We address the problem of coreset selection for realistic and challenging continual learning scenarios, where the data continuum is composed of class-imbalanced or noisy instances that deteriorate the performance of the continual learner during training.

\item We propose \emph{Online Coreset Selection (OCS)}, a simple yet effective online coreset selection method to obtain a representative and diverse subset that has a high affinity to the previous tasks from each minibatch during continual learning. Specifically, we present three gradient-based selection criteria to select the coreset for current task adaptation while mitigating catastrophic forgetting. 

\item We demonstrate that OCS is applicable to any rehearsal-based continual learning method and experimentally validate it on multiple benchmark scenarios, where it largely improves the performance of the base algorithms across various performance metrics.
\end{itemize}


==> 4_main_neurips.tex <==
\section{Rehearsal-based Continual Learning}\label{sec:sec3}
We consider learning a model over a sequence of tasks $\{\mathcal{T}_1,\ldots, \mathcal{T}_T\}=\mathcal{T}$ , where each task is composed of independently and identically distributed datapoints and their labels, such that task $\mathcal{T}_t$ includes $\mathcal{D}_{t} = \{\textbfit{x}_{t,n}, y_{t,n}\}^{N_t}_{n=1}\sim\mathcal{X}_t\times\mathcal{Y}_t$, where $N_t$ is the total number of data instances, and $\mathcal{X}_t\times\mathcal{Y}_t$ is an unknown data generating distribution. We assume that an arbitrary set of labels for task $\mathcal{T}_t$, $\mathbf{y}_t=\{y_{t,n}\}^{N_t}_{n=1}$ has unique classes, $\mathbf{y}_t\cap\mathbf{y}_k=\emptyset$, $\forall t\neq k$. In a standard continual learning scenario, the model learns a corresponding task at each step and $t$-th task is accessible at step $t$ only. Let neural network $f_{\Theta}:\mathcal{X}_{1:T}\rightarrow\mathcal{Y}_{1:T}$ be parameterized by a set of weights $\Theta=\{\theta_l\}^{L}_{l=1}$, where $L$ is the number of layers in the neural network. We define the training objective at step $t$ as follows: 
\begin{align}
\begin{split}
\small
\underset{\Theta}{\text{minimize}}~\sum^{N_t}_{n=1}\ell(f_{\Theta}(\textbfit{x}_{t,n}), y_{t,n}), 
\label{eq:basic}
\end{split}
\end{align}
where $\ell(\cdot)$ is any standard loss function (e.g., cross-entropy loss). The naive CL design cannot retain the knowledge of previous tasks and thus results in catastrophic forgetting. To tackle this problem, rehearsal-based methods~\citep{CuongN2018iclr,chaudhry2018efficient,titsias2019functional} update the model on a randomly sampled replay buffer $\mathcal{C}_k$ constructed from the previously observed tasks, where $\mathcal{C}_k=\{\textbfit{x}_{k,j}, y_{k,j}\}^{J_k}_{j=1}\sim\mathcal{D}_k,~\forall k<t$ and $J_k\ll N_k$. Consequently, the quality of the selected instances is essential for rehearsal-based continual learning. For example, some data instances can be more informative and representative than others to describe a task and improve model performance. In contrast, some data instances can degrade the model's memorization of previous tasks' knowledge. Therefore, obtaining the most beneficial examples for the target task is crucial for the success of rehearsal-based CL methods. 

To validate our hypothesis, we design a continual learning scenario with a sequence of two tasks, Permuted MNIST ($\mathcal{T}_1$) $\rightarrow$ MNIST ($\mathcal{T}_2$). After training on $\mathcal{T}_1$, we update the model parameters through a single backpropagation step using a data point from $\mathcal{T}_2$ and measure the test accuracy of all the corresponding classes and $\mathcal{T}_1$ performance degeneration. The results for all individual data points from $\mathcal{T}_2$ are described in~\Cref{fig:motiv_adaptation} and~\Cref{fig:motiv_forgetting} as box plots. The influence of each data point from $\mathcal{T}_2$ has a large disparity not only on the corresponding class accuracy but also on past task's average forgetting, which will further accumulate when trained on a large number of data points and tasks.

%\TBDD{Furthermore, existing methods do not incorporate the instances' similarity and diversity during the selection procedure, which is essential to minimize the catastrophic forgetting in continual learning.} Consequently, 
Based on this motivation, our objective is to select the data instances that can promote current task adaptation while minimizing catastrophic forgetting on the previous tasks. However, obtaining the most representative data points from the entire dataset is computationally expensive and intractable for online continual learning. Hence, we postulate and empirically validate a straightforward assumption to select a representative coreset for a target dataset. 

More formally, for a given subset $\mathcal{B}_t$, dataset $\mathcal{D}_t$, and $\epsilon > 0$, we state our assumption formally.
% we postulate and verify the following two assumptions to select a representative coreset for a target dataset $\mathcal{D}_t$:While 

\begin{assumption}
\label{assumption1}
The gradient of any arbitrary subset approximates the gradient of the whole dataset,
\begin{align}
\begin{split}
\small
\bigg|\frac{1}{N_t}\nabla f_{\Theta}(\mathcal{D}_t)-\frac{1}{|\mathcal{B}_t|}\nabla f_{\Theta}(\mathcal{B}_t)\bigg|\leq\epsilon.
\label{eq:assump2}
\end{split}
\end{align}
\end{assumption}

In principle, obtaining a representative subset from a large dataset is still computationally expensive; therefore, we consider a minibatch as an approximation of the whole dataset and select few representative data instances at each minibatch iteration. While the approximation quality depends on the dataset and minibatch size, we empirically validate that the above assumption generally holds across various minibatch sizes. In particular, we conduct an experiment on the MNIST dataset, where we measure the mean squared distance between the gradients of a batch and whole dataset per iteration in \Cref{fig:assumption1}. Notably, even the gradients of an arbitrary subset with a small-sized minibatch are similar to the whole dataset with a small $\epsilon$, and it is more evident when compared to the irrelevant gradients from a different dataset (Permuted MNIST).

Under~\Cref{assumption1}, we propose a selection criterion that selects the subset with the smallest possible~$\epsilon$. Specifically, we select the coreset that maximizes the gradient similarity between the representative instances and the target dataset. More formally:
% \begin{assumption}
% \label{assumption1}
% Given a neural network $f_{\Theta}$ parameterized by $\Theta$, representative data points have similar gradient vectors with the averaged gradients from all examples in a target dataset,
% \end{assumption}
% \vspace{-0.25in}
\begin{align}
\begin{split}
\small
\mathbf{u}^*=\underset{\mathbf{u}\in\mathbb{N}^\kappa}{\text{maximize}}~ \mathcal{S}\left(\frac{1}{N_t}\nabla f_{\Theta}\left(\mathcal{D}_t\right), \frac{1}{\kappa}\sum_{n\in\mathbf{u}}\nabla f_{\Theta}\left(\textbfit{x}_{t,n},y_{t,n}\right)\right),~~~\text{where}~\mathbf{u}=\{n:n\in\mathbb{N}_{<N_t}\},
\label{eq:assump1}
\end{split}
\end{align}

where $\mathcal{S}$ is any arbitrary similarity function and $\mathbf{u}^*$ is an index set that selects top-$\kappa$ informative samples without replacement. Consequently, the model iteratively updates the parameters to find the optimal local minima of the loss, and informative data points obtain similar gradient directions with the averaged gradients of the dataset. In the next section, we propose \emph{OCS} which consists of a simple similarity criterion to achieve this objective. However, similarity criterion is not sufficient to select the representative coreset for online continual learning; hence, we also propose our diversity and coreset affinity criteria to mitigate catastrophic forgetting.

%While the approximation quality depends on the dataset and minibatch size, we empirically observed that often used minibatch size is enough to approximate the target dataset (see Figure~\ref{fig:visualize}).
\input{materials/2_adap_and_forget}
\input{4_z1_first_task}
\input{4_z2_continual}


 %\TBDD{more description, Figure~\ref{fig:motivation} (c)}


==> 4_main_old.tex <==
\section{Rehearsal-based Continual Learning}\label{sec:sec3}
We consider a sequence of tasks $\{\mathcal{T}_1, \mathcal{T}_2, ..., \mathcal{T}_T\}=\mathcal{T}$ and each task $\mathcal{T}_t$ is composed of a pair of independently and identically distributed datapoints and their labels, $\mathcal{D}_{t}=\{\textbf{x}_{t,n},y_{t,n}\}^{N_t}_{n=1}\sim\mathcal{X}_t\times\mathcal{Y}_t$, where $N_t$ is the total amount of data instances for task $t$, and $\mathcal{X}_t\times\mathcal{Y}_t$ is an unknown data generating distribution. We assume that an arbitrary set of labels for task $t$, $\textbf{Y}_t=\{y_{t,n}\}^{N_t}_{n=1}$ has unique classes, $\textbf{Y}_t\cap\textbf{Y}_k=\emptyset$, $\forall t\neq k$. In a continual learning scenario, a model learns a corresponding task at each step; $t^{th}$ task is only accessible at step $t$. A neural network $f$ predicts targets corresponding data $f:\mathcal{X}_{1:T}\rightarrow\mathcal{Y}_{1:T}$, and is parameterized to a set of weights $\mathcal{W}=\{\textbf{W}_l\}^{L}_{l=1}$, where $L$ is the number of layers. We define a training objective at step $t$ as follows: 
\begin{align}
\begin{split}
\small
\underset{\mathcal{W}}{\text{minimize}}~\sum^{N_t}_{n=1}\ell(f(\textbf{x}_{t,n};\mathcal{W}), y_{t,n}), 
%\\ \text{s.t.}~\textbf{W}_l^\top\textbf{W}_l=\textbf{I},~~\forall, \textbf{W}_l\in\mathcal{W}^{(t)}
%\underset{\mathcal{W}}{\text{minimize}}~\sum^{N_t}_{i=1}\ell(f_{\mathcal{W}^{(t)}}(\textbf{x}^{(t)}_i; \mathcal{W}^{(t-1)}), y^{(t)}_i),
\label{eq:basic}
\end{split}
\end{align}
where $\ell(\cdot)$ is a loss function. The naive design of continual learning cannot retain the knowledge of previous tasks, thus results in the catastrophic forgetting. To tackle this problem, rehearsal-based methods~\cite{CuongN2018iclr,chaudhry2018efficient,titsias2019functional} update the model reflecting a randomly sampled replay buffer $\mathcal{C}_k$ given previous tasks, where $\mathcal{C}_k=\{\textbf{x}_{k,j}, y_{k,j}\}^{B_k}_{j=1}\sim\mathcal{D}_k~\forall k<t$ and $B_k\ll N_k$.
% \subsection{Beneficial data points to the task}\label{sec/assumption}

\input{materials/2_adap_and_forget}
However, the selected instances' quality is extremely important for rehearsal-based continual learning. Since some examples are more informative and representative than others to describe a task, obtaining the most beneficial examples for the target task is crucial for these methods' success. \TBDD{Additionally, some examples are more easy to ruin the memorization of past tasks' knowledge.} To validate our hypothesis, we design a continual learning scenario with a sequence of two tasks, Permuted MNIST ($\mathcal{T}_1$) $\rightarrow$ Rotated MNIST ($\mathcal{T}_2$). After training $\mathcal{T}_1$, we update model parameters through a single backpropagation step using a data point from $\mathcal{T}_2$ and measure the test accuracy of a corresponding class and $\mathcal{T}_1$ performance degeneration. The results for all individual data points from $\mathcal{T}_2$ are described in Figure~\ref{fig:motivation} (a-b) as box plots. Note that data points have a large disparity not only on target class performance but also on the past task's forgetting, which will be even accumulated during training.

% Some examples are more informative or representative than others to describe a task. Hence, obtaining the most beneficial examples to a target task is important to a rehearsal-based continual learning with experience replay that uses a small coreset to maintain the knowledge during future training. 
Furthermore, existing methods do not incorporate the instances' similarity and diversity during the selection procedure, which is essential to minimize the catastrophic forgetting in continual learning. Consequently, we postulate and verify the following assumptions to select a representative coreset:
\paragraph{Assumption 1.} \emph{Given a neural network $f_\mathcal{W}$ parameterized by $\mathcal{W}$, representative data points have similar gradient vectors with the averaged gradients from all examples in a target dataset,}
\begin{align}
\begin{split}
\small
\underset{\textbf{m}\in\mathbb{R}^{N_t}}{\text{arg~max}}~\mathcal{S}\left(\frac{1}{|N_t|}\nabla f_\mathcal{W}\left(\mathcal{D}_t\right), \frac{1}{\kappa}\sum^{N_t}_{n=1}m_{n}\cdot\nabla f_\mathcal{W}\left(\textbf{x}_{t,n},y_{t,n}\right)\right),~~~\text{s.t.}~\textbf{m}\in\{0,1\}^{N_t},~|\textbf{m}|=\kappa,
\label{eq:similarity}
\end{split}
\end{align}
where $\mathcal{S}$ is any similarity function and $\textbf{m}$ is an indicator vector which selects $\kappa$ informative data instances. The model iteratively updates the parameters to find the optimal local minima of the loss. As such, informative data points can obtain similar gradient directions with the averaged gradients of the dataset. 

\paragraph{Assumption 2.} \emph{The gradient of an arbitrary subset approximates the gradient of a whole dataset,}
\begin{align}
\begin{split}
\small
|\nabla f_\mathcal{W}(\mathcal{B}_t)-\nabla f_\mathcal{W}(\mathcal{D}_t)|\leq\epsilon, 
\label{eq:similarity}
\end{split}
\end{align}
where $\mathcal{B}_t$ is a subset of a dataset $\mathcal{D}_t$ and $\epsilon$ is a small positive constant. Since obtaining a representative subset from a large dataset is computationally expensive, we bypass the problem by considering a minibatch as an approximation of a whole dataset and selecting a small representative data instances at each minibatch training. 
While the approximation quality depends on the dataset and minibatch size, we empirically observed that often used minibatch size is enough to approximate the target dataset (see Figure~\ref{fig:visualize}). % \TBDD{(include empirical analysis)}%\TBDD{we empirically observe that less than $1\%$ of dataset perform good approximation as shown in Figure~\ref{fig:}.}

\input{4_z1_first_task}
\input{4_z2_continual}



==> 5_discuss.tex <==
\section{Collaborative training with Rehearsal-based CL}\label{sec/coresets}
Main contributions of our work are on the online beneficial minibatch selection in terms of current task adaptation and compatibility with past tasks, and constructing informative coresets as ingredients of rehearsal-based continual learning (CL). Hence, our work is easily combined with existing attractive CL methods. In this section, we briefly describe more algorithmic details of several works and usage of our online cherrypicker to them.

\textbf{Gradient Episodic Memory (GEM)} variants~\cite{lopez2017gradient,chaudhry2018efficient} introduce the additional regularization term preventing the increase of the replay buffer loss as follows:
\begin{align}
\begin{split}
\small
&\underset{\mathcal{W}}{\text{minimize}}~\ell(f_\mathcal{W}(\mathcal{D}_{t})),&&\text{s.t.}~\ell(f_\mathcal{W}(\mathcal{C}_{1:t-1}))\leq\ell(f_{\mathcal{W}^{(t-1)}}(\mathcal{C}_{1:t-1})),&
\label{eq:agem}
\end{split}
\end{align}

\begin{align}
\begin{split}
\small
\tilde{\nabla}f=\nabla f - \frac{\nabla f^\top \nabla f_{ref}}{\nabla f^\top_{ref}\nabla f_{ref}}\nabla f_{ref}
\label{eq:agem-constraint}
\end{split}
\end{align}

%\textbf{\TBDD{Orthogonal subspace projection.}} \cite{chaudhry2020continual}
\textbf{Mode-connectivity SGD}~\cite{mirzadeh2020linear} 

\begin{align}
\begin{split}
\small
\widehat{\mathcal{W}}^{(t)} = \underset{\mathcal{W}}{\text{arg min}} \sum_{\alpha\in[0,1]}[\ell_{t-1}(\widehat{\mathcal{W}}^{(t-1)}+\alpha(\mathcal{W}-\widehat{\mathcal{W}}^{(t-1)}))\\+\ell_{t}(\mathcal{W}^{(t)}+\alpha(\mathcal{W}-\mathcal{W}^{(t)}))],
\label{eq:mc-sgd}
\end{split}
\end{align}
where $\alpha$ is a hyperparameter for the line connection variety, consisted of several random values in $[0,1]$.

==> 8_z3_limitations.tex <==
\vspace{-0.1in}
\section{Limitations}\label{sup:sec:limitations}
\vspace{-0.1in}
Although our simple yet effective selection strategy improves the performance across various realistic continual learning scenarios, it is still far from the desirable performance. However, we believe that we have provided a novel insight into the utility of gradients for summarizing the dataset, which improves the current task adaptation and mitigates catastrophic forgetting. We hope that our work will lead to follow-up works that exploit our findings and develop methods, which are scalable to practical continual learning scenarios. Furthermore, our method is limited to supervised learning, where arriving data points require a large amount of annotated class labels. We leave the exploration of OCS for unsupervised data streams for future research.

%\sout{On the other hand, we construct the problem design under supervised learning scenarios, where arriving data points require sophisticatedly annotated class labels. While our OCS successfully tackles real-world applications like imbalanced or noisy supervised continual learning problems, unfortunately, unsupervised continual learning has been unsolved and left for future work.}

\section{Societal Impact}\label{sup:sec:societal}
\vspace{-0.07in}
%\sout{Our novel rehearsal-based continual learning method, \emph{Online Coreset Selection} (OCS), has a promising potential to lead selective sample training not only for the current task but also to be positive to past tasks. To this end, we directly reduce the threat of catastrophic forgetting during continual learning. OCS also brings laboratory-scale continual learning problems to the real world. We believe that OCS will lighten the importance of the online selection of helpful coreset during online continual learning on a sequence of tasks, including redundant, imbalanced, and noisy instances.}
In this paper, we introduce \emph{Online Coreset Selection}, a novel rehearsal-based continual learning method to select representative and diverse samples for online continual learning. Our proposed selection strategy is likely to have a high impact on continual learning as most of the existing methods do not select the coreset before the current task training, which can introduce bias in the model in the realistic continual learning scenarios. Additionally, our selective online training would be vital for memory-constrained applications such as surveillance systems, autonomous driving, social media, and e-commerce, where the data stream is often composed of biased and noisy samples and the system's security plays an essential role in the practicality of the system.

Regarding the risks of our proposed system, an adversary might try to deceive the privacy of the system given the knowledge of the coreset. To mitigate this, we encourage the research community to investigate the robustness of the rehearsal-based continual learning methods against membership inference and model stealing attacks to make the system exhaustive and robust to diverse attacks.



==> materials/2_instance_importance.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c c}
    \hspace{-0.45in}
        \includegraphics[height=2.5cm]{figures/variance.pdf} &\hspace{-0.35in}
        \includegraphics[height=2.5cm]{figures/loss.pdf} \\
        (a) Effect of a data point &
        (b) Approximation of $\textbf{w}^*$ \\
    \end{tabular}
    \vspace{-0.05in}
    \caption{\footnotesize \textbf{(a): Varying degree of adaptations among instances.} Training data points on CIFAR-$100$ have different abilities to adapt to target classes. We use a ResNet-$18$. \textbf{(b): Obtaining low loss surface using $\hat{B}^{(i)}$.} Beneficial mini-batch $\hat{B}^{(i)}$ for target task $\mathcal{T}$ avoids the interference and rapidly converges with better optima.}
    \label{fig:motivation}
    \vspace{-0.15in}
\end{figure}

==> materials/2_method_compaison_table.tex <==
\begin{table*}[t!]
\small
\captionof{table}{\footnotesize \textbf{TBD.}}
\vspace{-0.05in}
%\addtolength{\tabcolsep}{-2.8pt}  
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
% \hline 
% \hline 
\toprule
Method & Regularization & Minibatch Selection & Buffer Selection & Memorization \\
\midrule
%\checkmark & $-$ & $-$ & 
A-GEM & \checkmark & $-$ & $-$ & Reservoir\\
ICaRL & $-$ & $-$ & $-$ & \checkmark\\
Coreset selection & $-$ & $-$ & $-$ & \checkmark\\
GSS & $-$ & $-$ & $-$ & \checkmark\\
ER-MIR & $-$ & $-$ & \checkmark & Reservoir\\
Bilevel Opt. & \checkmark & $-$ & $-$ & Reservoir\\
MC-SGD & \checkmark & $-$ & $-$ & Reservoir\\
OCS & $-$ & \checkmark & $-$ & \checkmark\\
\bottomrule
\end{tabular}}
\end{table*}

==> materials/4_method_figure.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \includegraphics[height=3.2cm]{figures/placeholder.pdf} 
    % \vspace{-0.05in}
    \caption{\footnotesize \textbf{Coreset Selection Criteria}}
    \label{fig:motivation}
    \vspace{-0.1in}
\end{figure*}

==> materials/5_bal_stl_plot.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=6cm]{figures/bal-stl.pdf} \\
    \vspace{-0.15in}
    \caption{\footnotesize .}
    \vspace{-0.15in}
    \label{fig:bal-stl-plot}
\end{figure}

==> materials/5_imb_stl_bar.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=6cm]{figures/imbalance.pdf} \\
    \vspace{-0.15in}
    \caption{\footnotesize Per-class accuracy comparison of single task learning on imbalanced Rotated MNIST. $1^{st}$ and $6^{th}$ classes have about $10$ times the larger amount of training instances than others.}
    \vspace{-0.15in}
    \label{fig:imb-stl-bar}
\end{figure}

==> materials/5_imb_stl_table.tex <==
\begin{table}[h]
\tiny
\begin{center}
\caption{\small Performance of single task learning on imbalanced Rotated MNIST. The number of training instances at each class is $N_{c_{1:10}}:[\textbf{5920}, 670, 590, 610, 680, \textbf{5420}, 590, 620, 580, 590]$.}
\small
\begin{tabular}{c|c|cc}
\hline 
\hline 
%CherryPicker & Acc($c_{1:10}$) & Acc($c_1,c_6$) & Acc($c_{2:5},c_{7:10}$)\\
CherryPicker & Acc($c_{1:10}$) & Acc($c_{1,6}$) & Acc($c_{2:5,7:10}$)\\
\hline 
$\mathcal{S}_b - \mathcal{S}_c$ & \textbf{93.1 ($\pm$ 0.34)} & 98.6 ($\pm$ 0.64) & \textbf{91.7 ($\pm$ 0.38)}\\
$\mathcal{S}_b + \mathcal{S}_c$ & 90.5 ($\pm$ 0.80) & \textbf{99.1 ($\pm$ 0.25)} & 88.4 ($\pm$ 1.03)\\
$\mathcal{S}_r$ & 92.2 ($\pm$ 0.35) & 98.8 ($\pm$ 0.54) & 90.5 ($\pm$ 0.55)\\
$\mathcal{S}_c$ & 24.9 ($\pm$ 2.41) & 94.2 ($\pm$ 1.21) & ~~7.5 ($\pm$ 3.09)\\
\hline
Random & 87.5 ($\pm$ 1.40) & 97.7 ($\pm$ 0.76) & 85.0 ($\pm$ 1.91)\\
\hline \hline
  \end{tabular}
\label{tab:imbalanced_stl}
\vspace{-0.2in}
\end{center}
\end{table}


==> materials/5_imbalanced_dataset.tex <==
\begin{figure}
    \centering
    \includegraphics[width=5cm, height=3cm]{figures/class-distribution.pdf}\\
    \caption{\footnotesize \textbf{The number of training instances at each class.}}
    \label{fig:imbalanced-data}
    \vspace{-0.15in}
\end{figure}

==> materials/5_imbalanced_table.tex <==
\begin{table*}[t]
% 	\begin{minipage}[b]{0.50\linewidth}
% \begin{center}
% \caption{\small Evaluation on class-wise imbalanced-continual learning on Rotated MNIST dataset. We report tthe average accuracy (Accuracy) and average forgetting (Forgetting) across five independent runs. The best results are highlighted in bold.}
% \resizebox{\textwidth}{!}{%
% \addtolength{\tabcolsep}{-2.8pt}  
% \begin{tabular}{lcc cccc  cc}
% \toprule
% \multicolumn{1}{l}{{Method}}&\multicolumn{1}{c}{Accuracy}&\multicolumn{1}{c}{Forgetting}\\
% \midrule
% %MC-SGD~\cite{mirzadeh2020linear} &
% %{xx.x} \scriptsize{($\pm$ x.xx)} & {x.xx} \scriptsize{($\pm$ x.xx)} \\

% %Cherrypicker (Ours) &
% %{75.6} ($\pm$ 1.18) & {0.19} ($\pm$ 0.01) \\

% % Cherrypicker + MC-SGD (Ours) &
% %\textbf{{81.4} ($\pm$ 0.87)} & \textbf{{0.05} ($\pm$ 0.01)} \\

% %\midrule
% FINETUNE & 
% {xx.x} \scriptsize{($\pm$ x.xx)} & {x.xx} \scriptsize{($\pm$ x.xx)} \\

% A-GEM~\cite{chaudhry2018efficient}  &
% {xx.x} \scriptsize{($\pm$ x.xx)} & {x.xx} \scriptsize{($\pm$ x.xx)} \\

% ER-Reservior~\cite{chaudhry2019continual}  &
% {xx.x} \scriptsize{($\pm$ x.xx)} & {x.xx} \scriptsize{($\pm$ x.xx)} \\

% Stable SGD~\cite{mirzadeh2020understanding}  &
% {xx.x} \scriptsize{($\pm$ x.xx)} & {x.xx} \scriptsize{($\pm$ x.xx)} \\
% \midrule
% Uniform Sampling  &
% {61.6} \scriptsize{($\pm$ 1.72)} & {0.15} \scriptsize{($\pm$ 0.01)}  \\

% iCaRL~\cite{rebuffi2017icarl}  &
% {71.7} \scriptsize{($\pm$ 0.69)} & {0.09} \scriptsize{($\pm$ 0.00)} \\

% k-means features~\cite{CuongN2018iclr}  &
% {52.3} \scriptsize{($\pm$ 1.48)} & {0.24} \scriptsize{($\pm$ 0.01)}
% \\

% k-means embedding~\cite{csiba2018importance}  &
% {63.2} \scriptsize{($\pm$ 0.90)} & {0.13} \scriptsize{($\pm$ 0.02)} \\

% Grad Matching~\cite{campbell2019automated}  &
% {55.6} \scriptsize{($\pm$ 1.86)} & {0.18} \scriptsize{($\pm$ 0.02)} \\

% Bilevel Optim~\cite{borsos2020coresets}  &
% {xx.x} \scriptsize{($\pm$ x.xx)} & {x.xx} \scriptsize{($\pm$ x.xx)} \\

% \midrule
% ROCS (Ours) &
% \textbf{{76.5} \scriptsize{($\pm$ 0.84)}} & \textbf{{0.08} \scriptsize{($\pm$ 0.01)}} \\


%  \midrule
% MULTITASK & {xx.x} ($\pm$ x.xx) & $-$ \\
% % \hline \hline
% \bottomrule
% \end{tabular}}
% \label{tab:imbal_table}
% \vspace{-0.2in}
% \end{center}
% \end{table*}
% \end{minipage}\hfill
% \noindent
\begin{minipage}[b]{0.47\linewidth}
	\includegraphics[width=.49\textwidth]{figures/placeholder.pdf}
\includegraphics[width=.49\textwidth]{figures/placeholder.pdf}
% \includegraphics[width=.49\textwidth]{figures/adap.pdf}\hfill
% \includegraphics[width=.49\textwidth]{figures/fgt.pdf}\hfill 
\captionof{figure}{\small Evaluation on noisy balanced ({\bf left}) and imbalanced~({\bf right}) continual learning on Rotated MNIST dataset. The x-axis represents the degree of noise in the noisy dataset and y-axis represents the average accuracy across all the tasks across five independent runs. \label{fig:noisy_rot}}
\end{minipage}
\end{table*}

==> materials/5_interpolation.tex <==
%\setlength{\columnsep}{1pt}%
\begin{wrapfigure}{r}{0.3\linewidth}
    \centering
    \footnotesize
    \includegraphics[height=3.2cm]{figures/interpolation.pdf} 
    \caption{\footnotesize \textbf{Interpolation} TBD.}
    \label{fig:interpolation}
\end{wrapfigure}


==> materials/5_main_table_multiepoch.tex <==
\begin{table*}[t!]
\tiny
\begin{center}
\vspace{-0.1in}\caption{\small Performance comparison of the proposed method and other baselines on balanced and imbalanced continual learning. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across $5$ independent runs. The best results are highlighted in bold.}
\vspace{-0.1in}
\resizebox{\textwidth}{!}{%
\addtolength{\tabcolsep}{-2.8pt}  
\begin{tabular}{llc cccc  ccc}
% \hline 
% \hline 
\toprule
& {\textbf{Method}}&\multicolumn{2}{c}{\textbf{Rotated MNIST}} &\multicolumn{2}{c}{\textbf{Split CIFAR-100}}&\multicolumn{2}{c}{\textbf{Multiple Datasets}} \\
% \hline  \\
\midrule
& & Accuracy & Forgetting & Accuracy & Forgetting & Accuracy & Forgetting\\
\midrule
\parbox[t]{2mm}{\multirow{14}{*}{\rotatebox[origin=c]{90}{Balanced CL}}}
& FINETUNE & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& Stable SGD~\cite{mirzadeh2020understanding}  &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\
\cmidrule{2-9}
& Uniform Sampling &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 68.0} ($\pm$ 0.87) & {\scriptsize 0.13} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& iCaRL~\cite{rebuffi2017icarl} &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 69.1} ($\pm$ 0.77) & {\scriptsize 0.11} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& $k$-means Features~\cite{CuongN2018iclr} &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 66.7} ($\pm$ 1.28) & {\scriptsize 0.14} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& $k$-means Embedding~\cite{sener2018active}&
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 67.5} ($\pm$ 1.40) & {\scriptsize 0.13} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& Grad Matching~\cite{campbell2019automated} &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 68.1} ($\pm$ 0.88) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& ER-MIR~\cite{rahaf19ermir} &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

%& GSS~\cite{rahaf19gss} &
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

%& Bilevel Optim~\cite{borsos2020coresets} &
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

\cmidrule{2-9}

& OCS (Ours) &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 67.9} ($\pm$ 0.58) & {\scriptsize 0.13} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

\cmidrule{1-9}
%& MULTITASK & {\scriptsize 89.5} ($\pm$ 0.21) & $-$ & {\scriptsize 89.8} ($\pm$ 0.37) & $-$ & {\scriptsize 71.0} ($\pm$ 0.21) & $-$ \\
& MULTITASK & {\scriptsize 89.8} ($\pm$ 0.37) & $-$ & {\scriptsize 71.0} ($\pm$ 0.21) & $-$ & {\scriptsize 57.4} ($\pm$ 0.84) & $-$ \\
% \hline \hline
\midrule

\parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{Imbalanced CL}}}
& FINETUNE & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& Stable SGD~\cite{mirzadeh2020understanding}  &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\
\cmidrule{2-9}
& Uniform Sampling &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 58.3} ($\pm$ 1.65) & {\scriptsize 0.10} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& iCaRL~\cite{rebuffi2017icarl} &
{\scriptsize 61.5} ($\pm$ 0.95) & {\scriptsize 0.08} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& $k$-means Features~\cite{CuongN2018iclr} &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 59.7} ($\pm$ 2.62) & {\scriptsize 0.08} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& $k$-means Embedding~\cite{sener2018active}&
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 59.8} ($\pm$ 2.28) & {\scriptsize 0.09} ($\pm$ 0.01) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& Grad Matching~\cite{campbell2019automated} &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

& ER-MIR~\cite{rahaf19ermir} &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

%& GSS~\cite{rahaf19gss} &
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

%& Bilevel Optim~\cite{borsos2020coresets} &
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
%{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

\cmidrule{2-9}

& OCS (Ours) &
{\scriptsize xx.x} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx) & 
{\scriptsize 47.5} ($\pm$ 1.55) & {\scriptsize } ($\pm$ 0.14) & 
{\scriptsize 0.03} ($\pm$ x.xx) & {\scriptsize x.xx} ($\pm$ x.xx)\\

\cmidrule{1-9}
%& MULTITASK & {\scriptsize 89.5} ($\pm$ 0.21) & $-$ & {\scriptsize 89.8} ($\pm$ 0.37) & $-$ & {\scriptsize 71.0} ($\pm$ 0.21) & $-$ \\
& MULTITASK & {\scriptsize 81.0} ($\pm$ 0.95) & $-$ & {\scriptsize 48.2} ($\pm$ 0.72) & $-$ & {\scriptsize 41.4} ($\pm$ 0.97) & $-$\\
% \hline \hline
\bottomrule
.\end{tabular}}
\label{tab:main_table}
\vspace{-0.25in}
\end{center}
\end{table*}

==> materials/5_noisy_stl_table.tex <==
\begin{table}
\tiny
\begin{center}
\caption{\small Test Accuracy of single task learning on noisy Rotated MNIST. We vary the degree of the ratio of noise examples in the training dataset.}
\small
\begin{tabular}{c|c|c|c}
\hline 
\hline 
\multicolumn{1}{c|}{}&\multicolumn{3}{c}{\textbf{Method}}\\
\hline
\textbf{Noise} & \textbf{CherryPicker} & \textbf{Random} & \textbf{\TBDD{Remove Noise}} \\
\hline 
0\% & \textbf{97.8 ($\pm$ 0.20)} & 95.9 ($\pm$ 0.44) & 95.9 ($\pm$ 0.44)\\
20\% & \textbf{97.0 ($\pm$ 0.25)} & 93.3 ($\pm$ 0.58) & 95.4 ($\pm$ 0.22)\\
50\% & \textbf{93.7 ($\pm$ 0.33)} & 87.6 ($\pm$ 0.92) & \textbf{94.2 ($\pm$ 0.21)}\\
80\% & \textbf{80.0 ($\pm$ 2.36)} & 58.4 ($\pm$ 1.94) & \textbf{90.7 ($\pm$ 0.79)}\\
\hline \hline
  \end{tabular}
\label{tab:noisy_stl}
\vspace{-0.2in}
\end{center}
\end{table}

\begin{table}[h]
\tiny
\begin{center}
\caption{\small (temporal) Wallclock Time Comparison.}
\small
\begin{tabular}{c|c}
\hline 
\hline 
\textbf{CherryPicker} & \textbf{Random}\\
\hline 
34.1 s &  16.0 s \\
\hline \hline
  \end{tabular}
\label{tab:time}
\vspace{-0.2in}
\end{center}
\end{table}



==> materials/5_running_time.tex <==
\begin{wraptable}{r}{0.25\textwidth}
\tiny
\vspace{-1.1in}
\caption{\footnotesize TBD.}
\vspace{-0.1in}
\resizebox{0.25\textwidth}{!}{%
\addtolength{\tabcolsep}{-2.8pt}  
\begin{tabular}{cr}
% \hline 
% \hline 
\toprule
% \hline  \\
\midrule
Method & Training Time\\
\midrule
ER-MIR~\cite{aljundi2019online}& \TBDD{$~\text{h}~(\times0.7)$}\\
GSS~\cite{aljundi2019gradient}& \TBDD{$~\text{h}~(\times8.1)$}\\
Bi-Opt.~\cite{borsos2020coresets} & \TBDD{$12.1~\text{h}~(\times0.0)$}\\
OCS (Ours) & \TBDD{$2.9~\text{h}~(\times1.0)$} \\
\bottomrule
\end{tabular}}
\label{tab:time}
\vspace{-0.65in}
\end{wraptable}

==> materials/5_samples.tex <==
% \begin{figure*}[t!]
% \vspace{-0.05in}
% \begin{minipage}{0.48\linewidth}
% \captionof{table}{\footnotesize Ablation study on OCS selection.\label{fig:interpolation}}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{\hskip3pt}ccc cc@{\hskip3pt}}
% \toprule
% \multicolumn{1}{c}{Method}&\multicolumn{2}{c}{\textbf{Balanced Rotated MNIST}} & \multicolumn{2}{c}{\textbf{Balanced Rotated MNIST}}\\
% \midrule
% & Accuracy & Forgetting\\
% \midrule
% OCS-raw&72.7 \tiny{($\pm$ 0.47)}&0.13 \tiny{($\pm$ 0.01)}\\
% OCS-feat.&71.7 \tiny{($\pm$ 0.62)}&0.17 \tiny{($\pm$ 0.01)}\\
% OCS-grad.&\textbf{82.5 \tiny{($\pm$ 0.32)}}&\textbf{0.08 \tiny{($\pm$ 0.00)}}\\
% \bottomrule
% \end{tabular}}
% \begin{minipage}{0.5\linewidth}
% \includegraphics[width=\linewidth]{figures/interpolation.pdf}
% \captionof{figure}{\footnotesize Interpolation between $\mathcal{S}$ and $\mathcal{V}$.\label{fig:interpolation}}
% \end{minipage}%
% \begin{minipage}{0.5\linewidth}
% \captionof{table}{\footnotesize Running time on Rot-MNIST.\label{fig:interpolation}}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{cr}
% \toprule
% Method & Training Time\\
% \midrule
% ER-MIR~\cite{aljundi2019online}& \TBDD{$~\text{h}~(\times0.7)$}\\
% GSS~\cite{aljundi2019gradient}& \TBDD{$~\text{h}~(\times8.1)$}\\
% Bi-Opt.~\cite{borsos2020coresets} & \TBDD{$12.1~\text{h}~(\times0.0)$}\\
% OCS (Ours) & \TBDD{$2.9~\text{h}~(\times1.0)$} \\
% \bottomrule
% \end{tabular}}
% \vspace{-0.1in}
% \end{minipage}
% \end{minipage}%
% \hspace{0.05in}
% \begin{minipage}{0.5\linewidth}
%   \resizebox{\linewidth}{!}{%
%     \begin{tabular}{ccccc ccccc ccccc}
%         \includegraphics[height=1cm]{figures/coresets/uniform_0.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/uniform_1.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/uniform_2.pdf} & \hspace{-0.2in} 
%         % \includegraphics[height=1.05cm]{figures/coresets/uniform_3.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/uniform_4.pdf} & 
%         \includegraphics[height=1.05cm]{figures/coresets/icarl_2.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/icarl_6.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/icarl_4.pdf} & \hspace{-0.2in} 
%         % \includegraphics[height=1.05cm]{figures/coresets/icarl_1.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/icarl_9.pdf} & 
%         \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_5.pdf} &\hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_6.pdf} &\hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_7.pdf} &\hspace{-0.2in} 
%         % \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_8.pdf} &\hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_9.pdf} \\
%         \multicolumn{4}{c}{\textbf{(a) Uniform (imbalanced)}} & \multicolumn{4}{c}{\textbf{(b) iCaRL (imbalanced)}} & \multicolumn{4}{c}{\textbf{(c) Ours (imbalanced)}} \vspace{0.05in}\\
%         \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_0.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_1.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_2.pdf} & \hspace{-0.2in} 
%         % \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_3.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_4.pdf} & 
%         \includegraphics[height=1.05cm]{figures/coresets/icarl2_0.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/icarl2_3.pdf} & \hspace{-0.2in} 
%         % \includegraphics[height=1.05cm]{figures/coresets/icarl2_5.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/icarl2_7.pdf} & \hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/icarl2_8.pdf} & 
%         \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_0.pdf} &\hspace{-0.2in} 
%         %\includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_1.pdf} &\hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_3.pdf} &\hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_4.pdf} &\hspace{-0.2in} 
%         \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_2.pdf} \\
%         \multicolumn{4}{c}{\textbf{(d) Uniform (noisy)}} & \multicolumn{4}{c}{\textbf{(e) iCaRL (noisy)}} & \multicolumn{4}{c}{\textbf{(f) Ours (noisy)}} \\
%     \end{tabular}}
%     \vspace{-0.1in}
%     \caption{\footnotesize Randomly picked coreset examples. Top: Imbalanced Rot-MNIST. Bottom: $60\%$ Noisy Rot-MNIST.}
%     \label{fig:visualize}
% {\footnotesize
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccc}
% \includegraphics[width=1cm]{figures/tsne_blopt_run4_coreset_n200.png}&
% \includegraphics[width=1cm]{figures/tsne_blopt_run1_gss_greedy_n200.png}&
% \includegraphics[width=1cm]{figures/tsne_ocs_run3_fair_cherryset_n200.png}\\
% % \TBDD{{\tiny (a) Bilevel Optim}} & \TBDD{{\tiny (b) GSS}} & \TBDD{{\tiny (c) OCS (Ours)}} \\
% \end{tabular}}
% \vspace{-0.2in}
% \caption{\footnotesize T-SNE visualization of the selected samples.}
% \label{fig:tsne}}
% \end{minipage}
% \vspace{-0.27in}
% \end{figure*}
        

==> materials/5_samples_old.tex <==

\begin{figure*}[t!]
\vspace{-0.15in}
\begin{minipage}{0.48\linewidth}
\captionsetup{font=scriptsize}
\captionof{table}{\small Ablation study of our proposed method on imbalanced continual learning.}
\vspace{-0.1in}
\label{tab:ocs-ablation}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\hskip3pt}ccccc@{\hskip3pt}}
\toprule
\multicolumn{1}{c}{Method}&\multicolumn{2}{c}{\textbf{Balanced Rotated MNIST}} & \multicolumn{2}{c}{\textbf{Balanced Rotated MNIST}}\\
\midrule
& Accuracy & Forgetting & Accuracy & Forgetting\\
\midrule
OCS-raw&72.7 \tiny{($\pm$ 0.47)}&0.13 \tiny{($\pm$ 0.01)}\\
OCS-feat.&71.7 \tiny{($\pm$ 0.62)}&0.17 \tiny{($\pm$ 0.01)}\\
OCS-grad.&\textbf{82.5 \tiny{($\pm$ 0.32)}}&\textbf{0.08 \tiny{($\pm$ 0.00)}}\\
\bottomrule
\end{tabular}}
\end{minipage}\\
\begin{minipage}{0.48\linewidth}
 \centering
\vspace{-0.01in}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccccc ccccc ccccc}
        \includegraphics[height=1cm]{figures/coresets/uniform_0.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/uniform_1.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/uniform_2.pdf} & \hspace{-0.2in} 
        % \includegraphics[height=1.05cm]{figures/coresets/uniform_3.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/uniform_4.pdf} & 
        \includegraphics[height=1.05cm]{figures/coresets/icarl_2.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/icarl_6.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/icarl_4.pdf} & \hspace{-0.2in} 
        % \includegraphics[height=1.05cm]{figures/coresets/icarl_1.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/icarl_9.pdf} & 
        \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_5.pdf} &\hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_6.pdf} &\hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_7.pdf} &\hspace{-0.2in} 
        % \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_8.pdf} &\hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/fair_cherryset_9.pdf} \\
        \multicolumn{4}{c}{(a) Uniform (imbalanced)} & \multicolumn{4}{c}{(b) iCaRL (imbalanced)} & \multicolumn{4}{c}{(c) Ours (imbalanced)} \vspace{0.05in}\\
        \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_0.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_1.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_2.pdf} & \hspace{-0.2in} 
        % \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_3.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/imb_uniform_4.pdf} & 
        % \includegraphics[height=1.05cm]{figures/coresets/icarl2_5.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/icarl2_3.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/icarl2_0.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/icarl2_7.pdf} & \hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/icarl2_8.pdf} & 
        \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_0.pdf} &\hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_1.pdf} &\hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_2.pdf} &\hspace{-0.2in} 
        % \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_3.pdf} &\hspace{-0.2in} 
        \includegraphics[height=1.05cm]{figures/coresets/imb_fair_cherryset_4.pdf} \\
        \multicolumn{4}{c}{(d) Uniform Sampling (noisy)} & \multicolumn{4}{c}{(e) iCaRL (noisy)} & \multicolumn{4}{c}{(f) Ours (noisy)} \\
    \end{tabular}}
    \caption{\footnotesize \textbf{Coreset examples}. \textbf{Top row:} Visualization of coreset instances for imbalanced Rot-MNIST. \textbf{Bottom row:} Visualization of coreset instances on balanced Rot-MNIST with $60\%$ of random noisy instances. All samples are randomly picked.}
    \label{fig:visualize}
\end{minipage}%
\hspace{0.05in}
\begin{minipage}{0.5\linewidth}
\vspace{-0.8in}
\captionsetup{font=small}
{\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc}
\captionsetup{font=scriptsize}
\includegraphics[width=0.3\linewidth]{figures/tsne_kme_run5_kmeans_embedding_n200.png}
\vspace{-0.05in}&
\includegraphics[width=0.3\linewidth]{figures/tsne_blopt_run4_coreset_n200.png}&
\includegraphics[width=0.3\linewidth]{figures/tsne_blopt_run1_gss_greedy_n200.png}\\
  \multicolumn{1}{c}{(a) k-means} & \multicolumn{1}{c}{(b) Bilevel Opt.} & \multicolumn{1}{c}{(c) GSS} \\
\includegraphics[width=0.3\linewidth]{figures/tsne_ocs_sim_run4_fair_cherryset_n200.png}\vspace{-0.05in}&
\includegraphics[width=0.3\linewidth]{figures/tsne_ocs_div_run1_fair_cherryset_n200.png}&
\includegraphics[width=0.3\linewidth]{figures/tsne_ocs_run3_fair_cherryset_n200.png}\\
  \multicolumn{1}{c}{(d) $\mathcal{S}$ (Ours)} &\multicolumn{1}{c}{(e) $\mathcal{V}$ (Ours)} & \multicolumn{1}{c}{(f) OCS (Ours)} \\
% Ours-$\mathcal{S}_b$ & 
% \hspace{-0.15in}Ours-$\mathcal{V}$& 
% \hspace{-0.15in}\textbf{Ours}\\
\end{tabular}}
\caption{\footnotesize \textbf{T-SNE visualization of the selected samples}. Visualization of the selected samples by different baselines, our proposed selection criterions and OCS.}
    \label{fig:tsne}}
\end{minipage}
\vspace{-0.1in}
\end{figure*}


%\includegraphics[height=1cm]{figures/coresets/imb_icarl_0.pdf} & \hspace{-0.2in} 
%\includegraphics[height=1cm]{figures/coresets/imb_icarl_1.pdf} & \hspace{-0.2in} 
%\includegraphics[height=1cm]{figures/coresets/imb_icarl_2.pdf} & \hspace{-0.2in} 
%\includegraphics[height=1cm]{figures/coresets/imb_icarl_3.pdf} & \hspace{-0.2in} 
%\includegraphics[height=1cm]{figures/coresets/imb_icarl_4.pdf} & 
        

==> materials/8_bilevel_opt.tex <==
\begin{table}
\caption{\small Performance comparison with Bilevel Optimization method for balanced and imbalanced continual learning scenario. We perform five individual runs. We use TITAN Xp for training.}
\begin{tabular}{c ccc}
% \hline 
% \hline 
\toprule
\multicolumn{1}{c}{Method}&\multicolumn{3}{c}{\textbf{Balanced Rotated MNIST}}\\
% \hline  \\
\midrule
 & Accuracy & Forgetting & Wall-clock Time\\
\midrule
%\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\tiny Imbalanced}}}
Bilevel Opt. & 
80.7 \scriptsize{($\pm$ 0.44)} & 0.14 \scriptsize{($\pm$ 0.00)} & 12.1 h \\
OCS (Ours) &
\textbf{82.5 \scriptsize{($\pm$ 0.32)}} & \textbf{0.08 \scriptsize{($\pm$ 0.00)}} & 2.9 h\\
\midrule
\multicolumn{1}{c}{}&\multicolumn{3}{c}{\textbf{Imbalanced Rotated MNIST}}\\
% \hline  \\
\midrule
Method & Accuracy & Forgetting & Wall-clock Time\\
\midrule
Bilevel Opt. & 
57.3 \scriptsize{($\pm$ 0.35)} & 0.26 \scriptsize{($\pm$ 0.01)} & 10.5 h
\\
OCS (Ours) &
\textbf{76.5 \scriptsize{($\pm$ 0.84)}} & \textbf{0.08 \scriptsize{($\pm$ 0.01)}} & 1.6 h\\
\bottomrule
\end{tabular}
\label{sub:tab:bilevel}
\end{table}
%- \scriptsize{($\pm$ -)} & - \scriptsize{($\pm$ -)}
%\textbf{76.5 \scriptsize{($\pm$ 0.84)}} & \textbf{0.08 \scriptsize{($\pm$ 0.01)}} \\

==> materials/8_hyp_config.tex <==
%Stable SGD\vspace{-0.1in}
%\begin{itemize}
%    \item initial learning rate: [0.001, \textbf{0.005} (MNIST), 0.01, 0.05, \textbf{0.1} (Multiple), \textbf{0.15} (CIFAR), 0.5]
%    \item learning rate decay: [0.7, \textbf{0.75}, \textbf{0.8} (MNIST), 0.85, \textbf{0.875} (CIFAR, Multiple), 0.9]
%\end{itemize}
\TBDD{Uniform Sampling\vspace{-0.1in}
\begin{itemize}
    \item $\lambda$ (regularization):
\end{itemize}

iCaRL\vspace{-0.1in}
\begin{itemize}
    \item $\lambda$:
\end{itemize}

$k$-means Features\vspace{-0.1in}
\begin{itemize}
    \item $\lambda$:
\end{itemize}

$k$-means Embedding\vspace{-0.1in}
\begin{itemize}
    \item $\lambda$:
\end{itemize}

Grad Matching\vspace{-0.1in}
\begin{itemize}
    \item $\lambda$:
\end{itemize}
}
OCS (Ours)\vspace{-0.1in}
\begin{itemize}
    \item batch size: [\textbf{20} (CIFAR, Multiple), \textbf{100} (MNIST)]
    \item $\lambda$: [\textbf{0.05} (CIFAR), \textbf{0.1}, \textbf{1} (Multiple), \textbf{10}, \textbf{50} (MNIST)]
    \item $\tau$ : \textbf{1,000}
    %\item batch size: [\textbf{20} (CIFAR, Multiple), \textbf{100} (MNIST)]
    %\item $\lambda$ (regularization): [0.01, \textbf{0.05} (CIFAR), \textbf{0.1}, \textbf{1} (Multiple), \textbf{10}, \textbf{50} (MNIST), 100]
    %\item $\tau$ : [1, 10, 100, \textbf{1,000}, 5,000]
\end{itemize}


==> olds/4_z1_generative.tex <==
%- GMVAE
%- Orthogonal latent space
\subsection{Orthogonal Projection of Gaussian Mixture VAEs}
\label{sec/orthogonal}
We define a probabilistic generative model and insert orthogonal subspace projection across tasks which increments generative ability without task interference. 
\paragraph{Gaussian mixture variational autoencoder.}
We use a variational autoencoder~\cite{kingma2013auto} with a Gaussian mixture prior~\cite{dilokthanakul2016deep,yang2019deep}. Let a set of inputs $\{\textbf{x}^{(t)}_i\}^{N_t}_{i=1}\sim\mathcal{X}^{(t)}$ for task $t$ are drawn from Gaussian mixture, and $\textbf{z}^{(t)}\sim\mathcal{Z}^{(t)}$ is a latent representation drawn from the prior distribution. Then, our objective is to learn a function $e:\mathcal{Z}^{(t)}\times\bsy\Theta\rightarrow\mathcal{X}^{(t)}$, parameterized by $\bsy\theta\in\bsy\Theta$. The generative model is defined as follows:
\begin{align}
\begin{split}
\small
%\textbf{x}^{(t)}
p(\textbf{v}^{(t)};\bsy\pi^{(t)}) & = \prod^K_{k=1}\pi^{(t)}_k,\\
p(\textbf{z}^{(t)}|v^{(t)}_k=1) & =\mathcal{N}(\bsy\mu^{(t)}_k, \text{diag}({\bsy\sigma^{(t)}_k}^2)),\\
p_{\bsy\theta}(\textbf{x}^{(t)}|\textbf{z}^{(t)}) & = \mathcal{N}(e(\textbf{z}^{(t)};\bsy\theta),\lambda\textbf{I})
%p_{\bsy\theta}(\textbf{x}^{(t)}|\textbf{z}^{(t)}) & = \mathcal{N}(\bsy\mu^{(t)}_x,\lambda\textbf{I})
\label{eq:encoder}
\end{split}
\end{align}
where $\bsy\pi^{(t)}$ denotes a probability for task $t$ for Gaussian mixture components satisfies $\sum_{k=1}^K\pi^{(t)}_k=1$ and $\textbf{v}^{(t)}\in\{0,1\}^{K}$ is a corresponding indicator vector. $\bsy\mu$ and $\bsy\sigma$ denotes a mean and variance variables, respectively, $\lambda$ is a hyperparameter.

It is well-known that obtaining the posterior distribution $p(\textbf{z}^{(t)},\textbf{v}^{(t)}|\textbf{x}^{(t)})$ is computationally intractable, we approximate it as $q_{\bsy\phi}(\textbf{z}^{(t)},\textbf{v}^{(t)}|\textbf{x}^{(t)})$, parameterized by $\bsy\phi$:
% because it is impossible to compute all x to compute exact p(x) -> we sample a few of z which is likely to x, and compute p(x) from those. This means that we need a new function Q(z|X) which can take a value of X and give us a distribution over z values that are likely to produce X. Hopefully the space of z values that are likely under Q will be much smaller than the space of all z’s that are likely under the prior P(z). => minimize KL divergence: KL[Q(z)kP(z|X)]

\begin{align}
\begin{split}
\small
%q_{\bsy\phi}(\textbf{z}^{(t)},\textbf{v}^{(t)}|\textbf{x}^{(t)})&=q_{\bsy\phi}(\textbf{z}^{(t)},\textbf{v}^{(t)}|\textbf{x}^{(t)}),
%q_{\bsy\phi}(\textbf{z}^{(t)}|\textbf{x}^{(t)})
%\text{KL}[q(\textbf{z}^{(t)})||p(\textbf{z}^{(t)}|\textbf{x}^{(t)})]=\\\mathbb{E}_{\textbf{z}^{(t)}}[\text{log}~q(\textbf{z}^{(t)})-\text{log}~p(\textbf{x}^{(t)}|\textbf{z}^{(t)}) - \text{log}~p(\textbf{z}^{(t)})] + \text{log}~p(\textbf{x}^{(t)})
\text{log}~p(\textbf{x}^{(t)})-\text{KL}\left[q(\textbf{z}^{(t)}|\textbf{x}^{(t)})||p(\textbf{z}^{(t)}|\textbf{x}^{(t)})\right]=~~~~~~~~~~~~\\\mathbb{E}_{\textbf{z}^{(t)}}\left[\text{log}~p(\textbf{x}^{(t)}|\textbf{z}^{(t)})\right] - \text{KL}\left[{q(\textbf{z}^{(t)}|\textbf{x}^{(t)})}||{p(\textbf{z}^{(t)})}\right]
\label{eq:generator}
\end{split}
\end{align}
%left-hand side
% P(z|X) is not something we can compute analytically: it describes the values of z that are likely to give rise to a sample. Assuming we use an arbitrarily high-capacity model for Q(z|x), then Q(z|x) will hopefully actually match P(z|X), in which case this KLdivergence term will be zero, and we will be directly optimizing log P(X).
%right-hand side
% q(z|X)=N(z|\mu(X;\phi),\Sigma(X;\phi)). In practice, µ and Σ are again implemented via neural networks, and Σ is constrained to be a diagonal matrix.The last term—D [Q(z|X)kP(z)]—is now a KL-divergence between two multivariate Gaussian distributions, which can be computed in closed form as:

\begin{align}
\begin{split}
\small
%\mathbb{E}_{\textbf{x}^{(t)}\sim \mathcal{D}^{(t)}}[\log p(\textbf{X}^{(t)}) - \text{KL}[q(\textbf{z}^{(t)}|\textbf{X}^{(t)})||p(\textbf{z}^{(t)}|\textbf{X}^{(t)})]]= \\
%\mathbb{E}_{\textbf{x}^{(t)}\sim \mathcal{D}}[\mathbb{E}_{\textbf{z}^{(t)}\sim q}[\log p(\textbf{x}^{(t)}|\textbf{z}^{(t)})] - \text{KL}[q(\textbf{z}^{(t)}|\textbf{x}^{(t)})||p(\textbf{z}^{(t)})]].
\sum_{i=1}^{N_t}\mathbb{E}_{\textbf{z}_i^{(t)}\sim q_{\bsy\phi}(\textbf{z}_i^{(t)}|\textbf{x}_i^{(t)})}[\log p(\textbf{x}_i^{(t)}|\textbf{z}_i^{(t)})] - \text{KL}[q(\textbf{z}_i^{(t)}|\textbf{x}_i^{(t)})||p(\textbf{z}_i^{(t)})],
\\ \text{s.t.}~\textbf{\bsy\phi}_l^\top\textbf{\bsy\phi}_l=\textbf{I},~~\forall, \textbf{\bsy\phi}_l\in\mathcal{\bsy\phi}
\label{eq:generator2}
\end{split}
\end{align}
where $\textbf{I}\in\mathbb{R}^d$ is an identity matrix. For $\bsy\phi_l\in\mathbb{R}^{d_{out}\times d_{in}\times h\times w}$ in a convolutional layer, we flatten it to $\bsy\phi_l\in\mathbb{R}^{d_{out}\times(d_{in} \cdot h \cdot w)}$.

A projection matrix $J_t=\mathbb{R}^{k\times k}$ satisfies,
\begin{align}
\begin{split}
\small
J^\top_t J_t&=\textbf{I}, ~~\text{s.t. rank}(J_t)=r,\\
J^\top_t J_j&=\textbf{0}, ~~\forall~t\neq j,\\
\label{eq:projection}
\end{split}
\end{align}
where $r\ll k$.

\subsection{Nonparametric Expansion of Latent Subspace}\label{sec/nonparametric}

\begin{align}
\begin{split}
\small
\label{eq:nonparametric}
\end{split}
\end{align}

==> styles/math_commands.tex <==
% \usepackage{xcolor}
% \usepackage{amsmath,amsfonts,amssymb, amsthm}

%\newenvironment{proof}{\noindent{\bf Proof}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-sketch}{\noindent{\bf Sketch of Proof}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-idea}{\noindent{\bf Proof Idea}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-of-lemma}[1]{\noindent{\bf Proof of Lemma #1}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-attempt}{\noindent{\bf Proof Attempt}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proofof}[1]{\noindent{\bf Proof}
of #1:\hspace*{1em}}{\qed\bigskip}
\newenvironment{remark}{\noindent{\bf Remark}\hspace*{1em}}{\bigskip}

% Complex \xxx for making notes of things to do.  Use \xxx{...} for general
% notes, and \xxx[who]{...} if you want to blame someone in particular.
% Puts text in brackets and in bold font, and normally adds a marginpar
% with the text ``xxx'' so that it is easy to find.  On the other hand, if
% the comment is in a minipage, figure, or caption, the xxx goes in the text,
% because marginpars are not possible in these situations.
{\makeatletter
 \gdef\xxxmark{%
   \expandafter\ifx\csname @mpargs\endcsname\relax % in minipage?
     \expandafter\ifx\csname @captype\endcsname\relax % in figure/caption?
       \marginpar{\textcolor{red}{xxx~}}% not in a caption or minipage, can use marginpar
     \else
       \textcolor{red}{xxx~}% notice trailing space
     \fi
   \else
     \textcolor{red}{xxx~}% notice trailing space
   \fi}
 \gdef\xxx{\@ifnextchar[\xxx@lab\xxx@nolab}
 \long\gdef\xxx@lab[#1]#2{{\bf [\xxxmark \textcolor{red}{#2} ---{\sc #1}]}}
 \long\gdef\xxx@nolab#1{{\bf [\xxxmark \textcolor{red}{#1}]}}
}

%\usepackage[T1]{fontenc}
%\usepackage{fourier}
%\DeclareSymbolFont{calletters}{OMS}{cmsy}{m}{n}
%\DeclareSymbolFontAlphabet{\mathcal}{calletters}

\newcommand{\concat}{\mathbin{||}}
\newcommand{\protocol}{\mathbb{P}}

%fields and groups
\newcommand{\F}{\mathbb{F}}
\newcommand{\Fp}{\F_p}
\newcommand{\Fq}{\F_q}
\newcommand{\Ftwo}{\F_2}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Qbar}{\overline{\Q}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\Vs}{\mathbb{V}}
\newcommand{\Fbar}{\overline{\mathbb{F}}}

% \DeclareMathOperator*{\Exp}{\mathbb{E}}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\sgn}{sgn}
% \DeclareMathOperator*{\pruned}{pruned}
% \DeclareMathOperator*{\proj}{proj}

%vectors, etc.
\newcommand{\av}{\mathbf{a}} \newcommand{\cv}{\mathbf{c}}
%\newcommand{\dv}{\mathbf{d}} \newcommand{\ev}{\mathbf{e}}
\newcommand{\rv}{\mathbf{r}} \newcommand{\sv}{\mathbf{s}}
\newcommand{\tv}{\mathbf{t}} \newcommand{\uv}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}} \newcommand{\wv}{\mathbf{w}}
\newcommand{\xv}{\mathbf{x}} \newcommand{\yv}{\mathbf{y}}
\newcommand{\zv}{\mathbf{z}} \newcommand{\zerov}{\mathbf{0}}
\renewcommand{\AA}{\mathbf{A}} \newcommand{\BB}{\mathbf{B}}
\newcommand{\CC}{\mathbf{C}} \newcommand{\FF}{\mathbf{F}}
\newcommand{\MM}{\mathbf{M}} \newcommand{\RR}{\mathbf{R}}
\renewcommand{\SS}{\mathbf{S}} \newcommand{\TT}{\mathbf{T}}
\newcommand{\UU}{\mathbf{U}} \newcommand{\XX}{\mathbf{X}}
\newcommand{\YY}{\mathbf{Y}} \newcommand{\KK}{\mathbf{K}}
\newcommand{\A}{\mathcal{A}} \newcommand{\B}{\mathcal{B}}
\newcommand{\dash}{\mbox{---}}
\renewcommand{\O}{\mathcal{O}}
%\newcommand{\qq}{\mathfrak{q}}
\newcommand{\QQ}{\mathfrak{Q}}
\newcommand{\ZQ}{\Z_{q}}

\newcommand{\vk}{\mathbf{k}}
%\newcommand{\vu}{\mathbf{u}}

\newcommand{\todo}[1]{\noindent {\color{blue} {\footnotesize {\bf TODO}:~{#1}}}}

\newcommand{\mr}[1]{\ensuremath{\mathrm{{#1}}}}
\newcommand{\la}{\ensuremath{\leftarrow}}
\newcommand{\ra}{\ensuremath{\rightarrow}}
\newcommand{\ala}{\ensuremath{\ \la\ }}
\newcommand{\ara}{\ensuremath{\ \ra\ }}
\newcommand{\rf}{\ensuremath{\overset{\$}{\la}}}

\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}

% -- bold math symbols, for some reason --
\newcommand{\boldalpha}{\ensuremath{\boldsymbol{\alpha}}}
\newcommand{\boldchi}{\ensuremath{\boldsymbol{\chi}}}
\newcommand{\boldtau}{\ensuremath{{\boldsymbol{\tau}}}}
\newcommand{\boldstar}{\ensuremath{\mathbf{*}}}
\newcommand{\bolda}{\ensuremath{\mathbf{a}}}
\newcommand{\boldb}{\ensuremath{\mathbf{b}}}
\newcommand{\boldc}{\ensuremath{\mathbf{c}}}
\newcommand{\boldd}{\ensuremath{\mathbf{d}}}
\newcommand{\bolde}{\ensuremath{\mathbf{e}}}
\newcommand{\boldf}{\ensuremath{\mathbf{f}}}
\newcommand{\boldg}{\ensuremath{\mathbf{g}}}
\newcommand{\boldh}{\ensuremath{\mathbf{h}}}
\newcommand{\boldi}{\ensuremath{\mathbf{i}}}
\newcommand{\boldj}{\ensuremath{\mathbf{j}}}
\newcommand{\boldk}{\ensuremath{\mathbf{k}}}
\newcommand{\boldl}{\ensuremath{\mathbf{l}}}
\newcommand{\boldm}{\ensuremath{\mathbf{m}}}
\newcommand{\boldn}{\ensuremath{\mathbf{n}}}
\newcommand{\boldo}{\ensuremath{\mathbf{o}}}
\newcommand{\boldp}{\ensuremath{\mathbf{p}}}
\newcommand{\boldq}{\ensuremath{\mathbf{q}}}
\newcommand{\boldr}{\ensuremath{\mathbf{r}}}
\newcommand{\bolds}{\ensuremath{\mathbf{s}}}
\newcommand{\boldt}{\ensuremath{\mathbf{t}}}
\newcommand{\boldu}{\ensuremath{\mathbf{u}}}
\newcommand{\boldv}{\ensuremath{\mathbf{v}}}
\newcommand{\boldw}{\ensuremath{\mathbf{w}}}
\newcommand{\boldx}{{\ensuremath{\mathbf{x}}}}
\newcommand{\boldy}{\ensuremath{\mathbf{y}}}
\newcommand{\boldz}{\ensuremath{\mathbf{z}}}
\newcommand{\boldzero}{\ensuremath{\boldsymbol{0}}}
\newcommand{\boldone}{\ensuremath{\boldsymbol{1}}}
\newcommand{\boldpi}{\ensuremath{\boldsymbol{\pi}}}
\newcommand{\boldPi}{\ensuremath{\boldsymbol{\Pi}}}

% -- bold italic math symbols, for some reason --
\newcommand{\boldia}{\ensuremath{\boldsymbol{a}}}
\newcommand{\boldib}{\ensuremath{\boldsymbol{b}}}
\newcommand{\boldic}{\ensuremath{\boldsymbol{c}}}
\newcommand{\boldid}{\ensuremath{\boldsymbol{d}}}
\newcommand{\boldie}{\ensuremath{\boldsymbol{e}}}
\newcommand{\boldif}{\ensuremath{\boldsymbol{f}}}
\newcommand{\boldig}{\ensuremath{\boldsymbol{g}}}
\newcommand{\boldih}{\ensuremath{\boldsymbol{h}}}
\newcommand{\boldii}{\ensuremath{\boldsymbol{i}}}
\newcommand{\boldij}{\ensuremath{\boldsymbol{j}}}
\newcommand{\boldik}{\ensuremath{\boldsymbol{k}}}
\newcommand{\boldil}{\ensuremath{\boldsymbol{l}}}
\newcommand{\boldim}{\ensuremath{\boldsymbol{m}}}
\newcommand{\boldin}{\ensuremath{\boldsymbol{n}}}
\newcommand{\boldio}{\ensuremath{\boldsymbol{o}}}
\newcommand{\boldip}{\ensuremath{\boldsymbol{p}}}
\newcommand{\boldiq}{\ensuremath{\boldsymbol{q}}}
\newcommand{\boldir}{\ensuremath{\boldsymbol{r}}}
\newcommand{\boldis}{\ensuremath{\boldsymbol{s}}}
\newcommand{\boldit}{\ensuremath{\boldsymbol{t}}}
\newcommand{\boldiu}{\ensuremath{\boldsymbol{u}}}
\newcommand{\boldiv}{\ensuremath{\boldsymbol{v}}}
\newcommand{\boldiw}{\ensuremath{\boldsymbol{w}}}
\newcommand{\boldix}{\ensuremath{\boldsymbol{x}}}
\newcommand{\boldiy}{\ensuremath{\boldsymbol{y}}}
\newcommand{\boldiz}{\ensuremath{\boldsymbol{z}}}

\newcommand{\transpose}[1]{\ensuremath{{#1}^{\intercal}}}

\newcommand{\boldA}{\ensuremath{\mathbf{A}}}
\newcommand{\boldB}{\ensuremath{\mathbf{B}}}
\newcommand{\boldC}{\ensuremath{\mathbf{C}}}
\newcommand{\boldD}{\ensuremath{\mathbf{D}}}
\newcommand{\boldE}{\ensuremath{\mathbf{E}}}
\newcommand{\boldF}{\ensuremath{\mathbf{F}}}
\newcommand{\boldG}{\ensuremath{\mathbf{G}}}
\newcommand{\boldH}{\ensuremath{\mathbf{H}}}
\newcommand{\boldI}{\ensuremath{\mathbf{I}}}
\newcommand{\boldJ}{\ensuremath{\mathbf{J}}}
\newcommand{\boldK}{\ensuremath{\mathbf{K}}}
\newcommand{\boldL}{\ensuremath{\mathbf{L}}}
\newcommand{\boldM}{\ensuremath{\mathbf{M}}}
\newcommand{\boldN}{\ensuremath{\mathbf{N}}}
\newcommand{\boldO}{\ensuremath{\mathbf{O}}}
\newcommand{\boldP}{\ensuremath{\mathbf{P}}}
\newcommand{\boldQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\boldR}{\ensuremath{\mathbf{R}}}
\newcommand{\boldS}{\ensuremath{\mathbf{S}}}
\newcommand{\boldT}{\ensuremath{\mathbf{T}}}
\newcommand{\boldU}{\ensuremath{\mathbf{U}}}
\newcommand{\boldV}{\ensuremath{\mathbf{V}}}
\newcommand{\boldW}{\ensuremath{\mathbf{W}}}
\newcommand{\boldX}{\ensuremath{\mathbf{X}}}
\newcommand{\boldY}{\ensuremath{\mathbf{Y}}}
\newcommand{\boldZ}{\ensuremath{\mathbf{Z}}}

\newcommand{\deq}{\mathrel{\mathop:}=}
\newcommand{\zo}{\ensuremath{\{0,1\}}} % bits
\newcommand{\zon}{\ensuremath{\{0,1\}^n}} % bits

% Theorem definitions

% \theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem*{claims}{Claim}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{myremark}[theorem]{Remark}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{construction}[theorem]{Construction}

%% custom macros

\newcommand{\esm}[1]{\ensuremath{#1}}
\newcommand{\ms}[1]{\esm{\mathsf{#1}}}

\newcommand{\prg}{\ms{PRG}}
\newcommand{\prf}{\ms{PRF}}
\newcommand{\prp}{\ms{PRP}}
\newcommand{\enc}{\ms{Enc}}
\newcommand{\compute}{\ms{Compute}}
\newcommand{\verify}{\ms{Verify}}

\newcommand{\poly}{\esm{\mr{poly}}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\negl}{\esm{\mr{negl}}}

\newcommand{\ord}[1]{\esm{{#1}^{\mr{th}}}}

\newcommand{\hyb}{\ms{Hyb}}
\newcommand{\Funs}{\ms{Funs}}
\newcommand{\getsr}{\xleftarrow{\textsc{r}}}
\newcommand{\Unif}{\ms{Unif}}

\newcommand{\appc}{\stackrel{c}{\approx}}
\newcommand{\apps}{\stackrel{s}{\approx}}
%\newcommand{\abs}[1]{\left| #1 \right|}

\newcommand{\classP}{\ms{P}}
\newcommand{\classBPP}{\ms{BPP}}
\newcommand{\classNP}{\ms{NP}}
\newcommand{\Ppoly}{\ms{P}/\ms{poly}}
\newcommand{\NCone}{\ms{NC^1}}

\newcommand{\round}[1]{\left\lfloor #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\iprod}[1]{\left\langle #1 \right\rangle}
%\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\set}[1]{\left\{ #1 \right\}}

\newcommand{\Zp}{\Z_p}
\newcommand{\Zq}{\Z_q}

\newcommand{\subind}[2]{{#1}^{(#2)}}

\newcommand{\eqq}{\stackrel{?}{=}}

\newcommand{\Otilde}{\widetilde{O}}

\newcommand{\hc}{\ms{hc}}

\newcommand{\xstar}{x^*}
\newcommand{\ystar}{y^*}

\newcommand{\DDHAdv}{\ms{DDHAdv}}
\newcommand{\PRFAdv}{\ms{PRFAdv}}
\newcommand{\SCPRFAdv}{\ms{SC\hbox{-}PRFAdv}}

\newcommand{\ct}{\ms{ct}}

\newcommand{\view}{\ms{view}_{P,V^*}}
\newcommand{\viewHonest}{\ms{view}_{P,V}}
\newcommand{\Sim}{\calS}

\newcommand{\Am}{\mathbf{A}}

\newcommand{\SIS}{\ms{SIS}}
\newcommand{\ISIS}{\ms{ISIS}}
\newcommand{\LWE}{\ms{LWE}}
\newcommand{\mLWE}{\ms{MatrixLWE}}

\newcommand{\Sm}{\mathbf{S}}
\newcommand{\Em}{\mathbf{E}}
\newcommand{\Um}{\mathbf{U}}

\newcommand{\LWEadv}{\ms{LWEAdv}}
\newcommand{\mLWEadv}{\ms{MatrixLWEAdv}}
\newcommand{\SISadv}{\ms{SISAdv}}
\newcommand{\ISISadv}{\ms{ISISAdv}}

\newcommand{\bv}{\mathbf{b}}
\newcommand{\Bm}{\mathbf{B}}
\newcommand{\Rm}{\mathbf{R}}

\newcommand{\pro}[1]{\langle #1 \rangle}
\newcommand{\Comm}{\ms{Commit}}
\newcommand{\cSAT}{\ms{circuit}\text{-}\ms{SAT}}

\newcommand{\sk}{\ms{sk}}

\newcommand{\hin}{h_{\text{in}}}
\newcommand{\hout}{h_{\text{out}}}
\newcommand{\chin}{c_{\text{in}}}
\newcommand{\chout}{c_{\text{out}}}
\newcommand{\patches}{\texttt{patches}}
\newcommand{\FP}{\texttt{FP}}
\newcommand{\conv}{\texttt{Conv}}

\newcommand{\proctrust}{\calP_{T}}
\newcommand{\procuntrust}{\calP_{U}}

\newenvironment{myitemize}
{\begin{itemize}[leftmargin=5.5mm, itemsep=2pt, topsep=0pt]}
	{\end{itemize}}

\newenvironment{myenumerate}
{\begin{enumerate}[leftmargin=5.5mm, itemsep=1pt, topsep=0pt]}
	{\end{enumerate}}

\renewcommand{\wp}{\ \textnormal{w.p.}\ }

\newcommand{\sign}{\textrm{sign}}
\newcommand{\Bernoulli}[1]{\texttt{Bernoulli}(#1)}
\newcommand{\relu}{\textrm{ReLU}}
\newcommand{\xadv}{x_{\textrm{adv}}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\renewcommand{\vec}[1]{\mathbold{#1}}

\newcommand{\Var}{\operatorname{Var}}
\newcommand{\OPT}{\operatorname{OPT}}
